FedRDF: A Robust and Dynamic Aggregation Function against Poisoning Attacks in Federated Learning

Federated Learning (FL) represents a promising approach to typical privacy concerns associated with centralized Machine Learning (ML) deployments. Despite its well-known advantages, FL is vulnerable to security attacks such as Byzantine behaviors and poisoning attacks, which can significantly degrade model performance and hinder convergence. The effectiveness of existing approaches to mitigate complex attacks, such as median, trimmed mean, or Krum aggregation functions, has been only partially demonstrated in the case of specific attacks. Our study introduces a novel robust aggregation mechanism utilizing the Fourier Transform (FT), which is able to effectively handling sophisticated attacks without prior knowledge of the number of attackers. Employing this data technique, weights generated by FL clients are projected into the frequency domain to ascertain their density function, selecting the one exhibiting the highest frequency. Consequently, malicious clients' weights are excluded. Our proposed approach was tested against various model poisoning attacks, demonstrating superior performance over state-of-the-art aggregation methods.

==> introduction4.tex <==
\section{Introduction}

\IEEEPARstart{F}{ederated} Learning (FL) \cite{mcmahan2017communication} represents a decentralized approach to Machine Learning (ML) where data is not centralized for analysis in typical data centers. Instead, FL involves multiple clients, an aggregator (or set of aggregators). These clients collaboratively train an ML model using their datasets without sharing raw data; only the locally generated parameters are shared with the aggregator. This decentralized approach addresses key privacy challenges linked to centralized ML, aligning with General Data Protection Regulation (GDPR) principles \cite{goddard2017eu}. FL emerges as a promising solution for privacy concerns and mitigates delays associated with data sharing and processing in server-based model training \cite{rasha2023federated}. Consequently, FL finds applications across various domains such as finance, healthcare, smart cities \cite{matheu2022federated}, and cybersecurity \cite{campos2021evaluating} due to its wide utility.


The FL training process involves each client transmitting individual model updates or weights to the aggregator. The aggregator then combines these contributions using an \textit{aggregation function}, typically averaging the clients' weights and returning the result to clients each training round. However, similar to centralized ML, FL faces security threats, including Byzantine clients that behave unexpectedly. Specifically, \textit{poisoning attacks} aim to alter data or the weights shared by clients with the aggregator, degrading the model's performance and impeding convergence \cite{xia2023poisoning}. Prior studies confirm FL's vulnerability to these attacks \cite{baruch2019little}, particularly exposing weaknesses in the average function or FedAvg \cite{mcmahan2017communication} used for aggregation.In FL, model poisoning attacks involve malicious modifications to weights/gradients in each training round, as highlighted in our discussion in \cite{hernandez2023intrusion}. Notably, since data isn't shared, model poisoning encompasses the effects of data poisoning attacks, like dirty-label \cite{bhagoji2019analyzing}. To counter these attacks, robust aggregation functions have been proposed, such as median, trimmed mean \cite{yin2018byzantine}, or Krum \cite{blanchard2017machine}. However, most of these approaches, and subsequent works building upon them, primarily tackle simple poisoning attacks where attackers cannot collaborate. Furthermore, some proposals assume knowledge of the attacker count, which might not be feasible in real-world scenarios or against sophisticated attacks where compromised nodes change each training round.

Our robust aggregation method differs from prior approaches as it doesn't rely on knowing the attacker count or statistical methodologies. Instead, we leverage the Fourier Transform (FT) \cite{gray2012fourier} to convert weights sent in each round into the frequency domain, enabling the calculation of their density function. This allows us to select only weights with higher frequencies, excluding noise. We thoroughly evaluated our method against two model poisoning attacks: random weight generation by compromised clients and the collusive min-max attack \cite{shejwalkar2021manipulating}. Results indicate superior performance compared to traditional aggregation functions, effectively countering both attacks without additional complexity. Our FT-based approach includes a simple mechanism to identify Byzantine attackers each training round. When attackers are absent, leveraging FedAvg yields better results than robust aggregation functions. Thus, our approach, FedRDF, dynamically chooses between FedAvg and FT based on the presence of malicious clients, optimizing system effectiveness. In summary, our contributions include:
\begin{itemize}
    \item Design and implementation of a novel Fourier Transform-based robust aggregation function for model poisoning attacks

    \item Definition of a threat model and implementation of different attacks for the evaluation and analysis of the proposed approach 
    
    \item Dynamic aggregation strategy to alternate between FedAvg and the proposed FT-based method based on the detection of malicious clients

   \item Extensive performance evaluation demonstrating enhanced resistance against certain attacks compared with state-of-the-art approaches
\end{itemize}

The paper's organization is as follows: it starts with foundational concepts in Section \ref{sec:Preliminaries}, then explores related works in Section \ref{related} focusing on robust aggregation against attacks. Section \ref{sec:Setup} outlines the threat model and considered attacks. Following this, Section \ref{sec:methodology} details the robust aggregation steps and dynamic client selection. The evaluation results are presented in Section \ref{sec:evaluation}, and finally, Section \ref{sec:conclution} summarizes the study's findings and conclusions.

%The rest of the paper is organized as follows: Section \ref{sec:Preliminaries} delineates the foundational concepts underpinning our work. Section \ref{related} describes other works related to the definition of robust aggregation functions to deal with poisoning attacks. Then, Section \ref{sec:Setup} describes the threat model, as well as the attacks considered in our work. Section \ref{sec:methodology} details the steps involved in our robust aggregation function and the dynamic selection based on the presence of malicious clients. The, Section \ref{sec:evaluation} describes the evaluation results. Finally, Section \ref{sec:conclution} summarizes the findings and conclusions drawn from our study.






==> methodology3.tex <==
\section{Methodology}\label{sec:methodology}
This section outlines our Byzantine-resilient secure aggregation function based on the FFT. The FFT possesses the inherent capability of deriving the density function through its frequency domain \cite{nanbu1995fourier}. To aggregate clients' weights using the FFT, upon receiving the weights $(W^k)_1^K$ from the $K$ clients, the server calculates the FFT in a coordinate-wise manner, and select the point of highest frequency, i.e., the highest density. In detail, as illustrated in Fig. \ref{fig:coorwise}, we compute vectors $V_{i,l} = {w^1_{i,l}, \dots, w^K_{i,l} }$, where $w^k_{i,l}$ represents the $i$-th element of the weights $W^k$ at layer $l$ of client $k$. Subsequently, these vectors $V_{i,l}$ are sorted. For each $i$ and $l$, we compute the FFT of this vector, transforming it into a frequency vector. This transformation is possible by projecting any function into the frequency domain, as discussed in Section \ref{sec:fourier}. Finally, we take the index of the maximum point of $FFT(V_{i,l})$, and select the corresponding point of $V_{i,l}$. Specifically, we take:
\begin{equation}\label{eq:fourierfinal}
    \Bar{w}_{i,l} = arg\, max_{w^k_{i,l}}\{FFT(V_{i,l})\} \forall i,l
\end{equation}

\begin{figure*} [!ht]
	\centering
		\includegraphics[scale = 0.8]{imagenes/System formulation/coorwise.pdf}
	\caption{Visual description of our aggregation method}
	\label{fig:coorwise}
\end{figure*}


The aggregated model, denoted as $\Bar{W}$, is obtained by consolidating all $\Bar{w}{i,l}$, and is then sent to the clients. The method relies on the principle that benign clients' weights tend to cluster closely in vector space.  High-density regions in the density function will indicate where benign weights congregate. Malicious weights, for impacting performance adversely, will deviate and be isolated from these high-density zones. By using FFT to compute the density function of the vector $V{i,l}$, we can identify these clusters. As a result, outlier weights exert minimal influence on the outcome of Equation \ref{eq:fourierfinal}, regardless of their magnitudes. 

This approach effectively shields the system from malicious clients. However, in scenarios without malicious activity, a simple mean of the weights proves most efficient (Section \ref{related} and further in our work). Current methods prioritize defense against spurious weights at the expense of some accuracy. To address this, our approach dynamically selects between the mean and Equation \ref{eq:fourierfinal}. This adaptability ensures minimal accuracy loss, using FedAvg in non-malicious settings and shifting to FFT-based aggregation with increased malicious client presence.

To optimize the final accuracy of the model and judiciously select between the two aggregation methods, we employ the Kolmogorov–Smirnov (K-S) test \cite{berger2014kolmogorov}, as outlined in \ref{alg:pseudocode}. The K-S test is a robust, non-parametric method for assessing the goodness-of-fit. This test contrasts two sample distributions to determine if they significantly diverge from one another. The essence of the K-S test is captured by the following equation:
\begin{equation}
    KS(F_1,F_2) = sup{F_1(x) - F_2(x)}
\end{equation}

where $F1$ and $F2$ are the cumulative distribution functions of the two samples under comparison, and $sup$ denotes the maximum difference between these distributions. By applying this test, we can effectively discern between benign and potentially  malicious weight distributions.%, thereby guiding the decision to use either of the aggregation methods to improve the model's performance.

%To test the latter assumption of benign weights will exhibit a consistent distribution pattern, we select a subset of points $\hat{V_{i,l}}$ of size $S$ from the vectors $V_{i,l}$ and calculate the $p$-value from the K–S test between $\hat{V_{i,l}}$ and $V_{i,l}\setminus \hat{V}_{i,l}$. A $p$-value exceeding 0.05 indicates that the sampled subset adheres to the general distribution of the remaining points, suggesting the absence of malign influences. Conversely, a lower $p$-value implies a deviation from the expected distribution, signaling the presence of potentially malicious clients. This testing procedure is replicated $C$ times for each vector $V_{i,l}$, with each iteration considering a different subset. We then compute the frequency with which the test results indicate a deviation from the expected distribution. The mean of these frequencies is calculated for every $i$ and $l$ of $V_{i,l}$. If this average $p$ surpasses a predetermined threshold $\alpha$, it implies the presence of malicious weights, prompting the server to implement the FFT for aggregation. If the average $p$ remains below $\alpha$, the server defaults to using FedAvg. A concise overview of this process is depicted in \ref{eq:trozos}, where $F$ represents the server's aggregation function.

To assess the consistency of benign weights' distribution, we select a subset $\hat{V_{i,l}}$ of size $S$ from vectors $V_{i,l}$. The $p$-value from the K–S test between $\hat{V_{i,l}}$ and $V_{i,l}\setminus \hat{V}_{i,l}$ indicates if the distribution of the two functions are equal. A $p$-value above 0.05 suggests alignment, signaling an absence of malign influences; and a lower $p$-value implies outliers in the distribution, leading potential malicious presence. This process is repeated $C$ times to add consistency, calculating the mean frequency of deviations for each $i$ and $l$. If this average $p$ surpasses a threshold $\alpha$, indicating malicious weights, the server switches to FFT for aggregation. If below $\alpha$, the server defaults to using FedAvg, since the is no malicious presence. Equation \ref{eq:trozos} summarizes this process, where $F$ is the server's aggregation function.



\begin{equation}\label{eq:trozos}
    F(W^1,\dots,W^K)= \left\{ \begin{array}{lcc}
                FedAvg(W^1,\dots,W^K) & if & p \leq \alpha  \\ \\ 
                FFT(W^1,\dots,W^K)& if &p > \alpha  \end{array} \right.
\end{equation}


This methodology optimizes performance regardless of malicious client count and fortifies against sudden attacks. For instance, if the system is secure up to round $r$, it employs FedAvg. Upon the onset of an attack at round $r+1$, it will switch to FFT for aggregation. This adaptive strategy aligns our method with the most effective function for each circumstance, avoiding unnecessary accuracy loss.

\begin{algorithm}%[H]
\caption{Algorithm of our robust dynamic federated learning framework}
\label{alg:pseudocode}
\begin{algorithmic}[1]
\REQUIRE $N$ set of clients, $R$ number of rounds, $E$ number of epochs, $C$ number of repetitions of malicious test, $S$ size of the subset part of malicious test, and $t$ threshold.

\ENSURE Global model $W$ \\

\FOR{$r$ in 1 to $R$}
    \STATE $W_r^k = \text{localUpdate}(W_{r-1},E)$
    \STATE Send $W_r^k$ to the server


\vspace{5pt}
\FOR{client $\in N$} 
    \STATE $W_r^k = \text{localUpdate}(W_{r-1},E)$ 
    \STATE Send $W_r^k$ to the server
\ENDFOR

\vspace{5pt}
\FOR{Server}
    \STATE $t_r = \text{mean}(Mal\_test(\{W_r^1,\dots,W_r^{|N|}\}), C, S)$ 
    \IF{$t_r < t$}
        \STATE $W_r = \text{mean}(\{W_r^1,\dots,W_r^{|N|}\})$
    \ELSE
        \STATE $W_r = \text{FFT}(\{W_r^1,\dots,W_r^{|N|}\})$  
    \ENDIF
    \STATE Send $W_r$ to clients
\ENDFOR

\ENDFOR


\vspace{7pt}
$Mal\_test(\{W_r^1,\dots,W_r^{|N|}\}), C, S):$
\STATE Calculate $V_{i,l} = \{w^1_{i,l}, \dots, w^K_{i,l} \}\forall i,l$
\FORALL{$V_{i,l}$}
\FOR{1, 2, \dots, C}
\STATE Take sample $\hat{V}_{i,l}$ of $V_{i,l}$ of size S 
\STATE Calculate $p$-value of $KS(\hat{V}_{i,l}, V_{i,l}\setminus \hat{V}_{i,l})$
\ENDFOR \hfill \break
\STATE Calculate average of the previous $p$-values
\ENDFOR \hfill \break
\STATE Return vector of $p$-values


\end{algorithmic}
\end{algorithm}

















\iffalse
The methods compare in our work first is fedProx [ref], a well kown method designing to deal with non-iid data.
\begin{equation}\label{eq:fedprox}
    W^{r+1} = \theta(W^r + \nu \nabla f(W^r))+(1-\theta)Average(W^r)
\end{equation}
Our method is based in equation \ref{eq:fedprox}, substituting the average by the weighted median.
\begin{equation}\label{eq:ourmethod}
    W^{r+1} = \theta(W^r + \nu \nabla f(W^r))+(1-\theta)WMedian(W^r)
\end{equation}

Future tests, use the absolute skeweness to test the dispersion of the data to dinamicaly choose between the mean and the median.
\begin{equation}\label{eq:totalSkewness}
    \frac{E(|X-E(X)|^3)}{Var(X)^{\frac{3}{2}}}
\end{equation}
\fi



==> system3.tex <==
\section{Threat model and considered attacks} \label{sec:Setup}
In this section, we describe the attacks considered in this work, and then, we will describe the complete FL system involving benign and malign clients.

\subsection{Threat model}
In Section \ref{sec:Preliminaries}, the considered FL scenarios are detailed, including attacks used to test our robust aggregation. We focus on a scenario with K clients and one aggregator. While we address a single aggregator, our method applies to decentralized or hierarchical setups with multiple aggregators \cite{lalitha2018fully}. Our threat model involves M compromised clients or byzantine attackers ($M < K/2$), assuming the aggregator remains uncompromised. Malicious clients ($m \in M$) execute one of two specified attacks in each assessment, detailed in the subsequent subsection.

To describe our threat model, we consider the systematization of threat models for poisoning attacks in FL proposed by \cite{shejwalkar2022back}. This system describes different aspects related to the characteristics of the attackers, including their objectives, knowledge, and capabilities:

\begin{itemize}
    \item \textbf{Adversary's Objective}: Both attacks aim to reduce model accuracy by manipulating locally generated weights in each FL round. These attacks are \textit{indiscriminate} or \textit{untargeted} \cite{baruch2019little} and \textit{generic}, causing general misclassification without specific class targeting.
    \item \textbf{Adversary's Knowledge}: Attackers access only their controlled client's updates, lacking access to other clients' data. However, in the min-max attack (Section \ref{sec:attacks}), compromised nodes collude using updates from other malicious nodes, indicating \textit{whitebox} knowledge \cite{shejwalkar2022back} of benign clients' models. Future consideration for attackers' knowledge of the aggregation function is planned.
    \item \textbf{Capabilities of the adversary}: Attacks poison client-generated models each training round. Access methods include direct device access or Man-in-the-middle attacks altering updates before sent to the aggregator. Both attacks follows an \textit{online} mode, occurring in each training round, unlike label-flipping attacks at training start. In the min-max attack, attackers collude with each other  exchanging updates to amplify impact.

    
\end{itemize}

Additionally, we assume a scenario with no dropouts or \textit{stragglers} \cite{park2021sageflow}, meaning the nodes remain active throughout all the rounds of the training process.


\subsection{Attacks considered}\label{sec:attacks}
Before presenting our FL robust aggregation approach, we introduce the considered attacks. In each training round, a node may be compromised, aiming to degrade the global model's performance. The first attack involves sending random weights instead of updated weights based on local training. Specifically, a compromised node transmits a set of weights randomly generated through Gaussian initialization (from the Keras library \cite{chollet2015keras}) to the aggregator. Despite their simplicity, these attacks, as demonstrated in prior works \cite{pillutla2022robust}, cause significant performance degradation without appropriate countermeasures.

The second type of attack is introduced in \cite{shejwalkar2021manipulating}, where the authors test some of the robust aggregation functions described in Section \ref{sec:Preliminaries},  exploiting weaknesses to reduce overall performance. Various attack strategies are categorized, and we adopt a challenging variant: the agnostic \textit{min-max} attack. This strategy remains effective even without knowledge of the aggregation function or benign clients' weights. Focusing on the \textit{min-max} attack is justified by \cite{shejwalkar2021manipulating} due to its more substantial impact compared to other attacks like LIE \cite{baruch2019little} and Fang \cite{fang2020local}.

The min-max attack methodology begins with malicious clients training models using a standard dataset akin to benign clients. These malign entities then exchange their computed weights among themselves. Subsequently, new weights are computed to maximize divergence from both the aggregated benign weights and each other's weights while maintaining subtlety to evade detection. These refined weights are transmitted to the aggregator. Equation \eqref{eq:minmax} illustrates the formulation:
\begin{equation}
    \label{eq:minmax}
    \Theta= A((W^m)_{m\in M}) + \gamma\Theta^p,
\end{equation}

Here, $M$ signifies the set of malicious clients, $A(\cdot)$ denotes the aggregation function, $\Theta^p$ represents the perturbation vector (direction), and $\gamma$ scales the perturbation added to the average malicious client weights (distance). $\gamma$ are calculated by Equation \eqref{eq:minmax2}. $\Theta^p$ can be derived through different methods \cite{shejwalkar2021manipulating}: using the inverse unit vector $-\frac{\Theta}{||\Theta||_2}$, inverse standard deviation, or inverse sign (the sign of the value). This work utilizes the inverse unit vector method due to its substantial impact on global model accuracy compare to the others. Figure \ref{fig:minmax} visually depicts the min-max attack: red points denote malicious weights, solid green represents benign weights, post-training weights of the malicious client are green with a red dot, and light green points signify hypothetical benign weights without malign influence. These malicious weights strategically position themselves as distant as feasible from benign weights, incrementally causing divergence to reduce the global model's accuracy. After training, malign clients share their weights to calculate the mean, and by Equation \eqref{eq:minmax}, derive the final malign weights sent to the server.

\begin{equation}
    \label{eq:minmax2}
    argmax_{\gamma} \max_{m\in M} ||\Theta -W^m|| \leq \max_{m,l \in M}  ||W^m - W^l||
\end{equation}

\begin{figure*} [!ht]
	\centering
		\includegraphics[width=1.7\columnwidth]{imagenes/System formulation/min-max.pdf}
	\caption{Visual description of how min-max attack works. The malicious weights (red points) separate from legitimate weights (green points), with the intention of degrading the overall system performance. The attack forces the legitimate weights to deviate from their true positions (indicated by light green), which they would naturally converge to in the absence of malicious entities.}
	\label{fig:minmax}
\end{figure*}

%The resulting FL scheme considered in this work is shown in Figure \ref{fig:FLsetup} with $K$ clients where there are $M<K$ compromised clients. These clients will send fake weights with the intention of harming the model performance, deviating the benign weights from their original direction. In some cases, malicious clients may operate independently (e.g., sending random weights) or collaborate to maximize their impact (e.g., through the min-max attack). Particularly in scenarios where several clients collude, as illustrated in Fig. \ref{fig:FLsetup}, certain clients join forces to generate certain weights aimed at significantly disrupting the overall process. This collaboration involves employing a specific function, denoted as $F_M$, which in our context refers to the min-max attack (see Equation \ref{eq:minmax}). 

This work's FL setup, depicted in Figure \ref{fig:FLsetup}, involves $K$ clients where there are $M<K/2$ compromised clients. These compromised clients aim to harm model performance by sending fake weights, shifting the benign weights from their original direction. Malicious clients may act independently (e.g., sending random weights) or collaborate to amplify their impact, as with the min-max attack. In scenarios where clients collude (as shown in Fig. \ref{fig:FLsetup}), they unite to generate disruptive weights, employing a specific function denoted as $F_M$, here referring to the min-max attack (Equation \ref{eq:minmax}).

\begin{figure} [!ht]
	\centering
		\includegraphics[width=0.8\columnwidth]{imagenes/System formulation/FedRDF.pdf}
	\caption{Scheme of our federated environment. Benign weights are presented as green packages. Malign clients cooperate to send malicious weights (red packages) to the server using a certain function $F_M$ (\ref{eq:minmax} in our case). The server aggregates the weights using a certain aggregation function $F$}
	\label{fig:FLsetup}
\end{figure}


